Opacity Proof for CaPR+ Algorithm

In this paper, we describe an enhanced Automatic Check- pointing and Partial Rollback algorithm(CaP R + ) to realize Software Transactional Memory(STM) that is based on con- tinuous conflict detection, lazy versioning with automatic checkpointing, and partial rollback. Further, we provide a proof of correctness of CaP R+ algorithm, in particular, Opacity, a STM correctness criterion, that precisely captures the intuitive correctness guarantees required of transactional memories. The algorithm provides a natural way to realize a hybrid system of pure aborts and partial rollbacks. We have also implemented the algorithm, and shown its effectiveness with reference to the Red-black tree micro-benchmark and STAMP benchmarks. The results obtained demonstrate the effectiveness of the Partial Rollback mechanism over pure abort mechanisms, particularly in applications consisting of large transaction lengths.

==> bib1.tex <==



\begin{thebibliography}{1}

% \bibitem{PTM}
%  Rachid Guerraoui, Michael Kapalka, “Principles of Transactional Memory”, \emph{Morgan \& Claypool publishers}, 2010. 
% \bibitem{TM} 
%  Tim Harris, James Larus and Ravi Rajwar, “Transactional Memory”, 2nd edition, \emph{Morgan \& Claypool publishers}, 2010.
% \bibitem{TMarch}
%  M. Herlihy and J. E. B. Moss. “Transactional memory: architectural support for lock-free data structures”. In Proc. of the \emph{Twentieth Annual International Symposium on Computer Architecture}, pp. 289–300, San Diego, California, 1993, ACM Press.
\bibitem{STM}
 N. Shavit and D. Touitou. `Software transactional memory`. \emph{In Distributed Computing}, Special Issue (10):99–116, 1997.
%\bibitem{hybrid}
% S. Kumar, M. Chu, et al, ``Hybrid transactional memory'', In Proceedings of the \emph{eleventh ACM SIGPLAN symposium on Principles
% and practice of parallel programming, PPoPP’ 06}, ACM Press, New York, NY, USA, March 2006.
% \bibitem{intel}
%  http://software.intel.com/en-us/articles/intel-c-stm-compiler-prototype-edition-20/
% \bibitem{version}
%  João Cachopo and António Rito-Silva. “Versioned boxes as the basis for memory transactions”, \emph{SCOOL’05: Proc. OOPSLAWorkshop on Synchronization and Concurrency in Object-Oriented Languages}, October 2005.
\bibitem{KuzPer:CORR:NI:2012}
Petr Kuznetsov and Sathya Peri. On non-interference of transactions. CoRR, abs/1211.6315, 2012% \bibitem{xlcstm}
%  http://www.alphaworks.ibm.com/tech/xlcstm.
\bibitem{checkpt}
 Koskinen E and Herlihy M, ``Checkpoints and continuations instead of nested transactions''. In
  Proceedings of the \emph{Twentieth annual symposium on Parallelism in algorithms and architectures (SPAA’08)}
(New York, NY, USA, 2008), ACM, pp. 160–168
\bibitem{lupei}
Lupei, D.: A study of conflict detection in software transactional memory. Master’s thesis, University of Toronto, the Netherlands (2009)
\bibitem{monika2}
Gupta, M., Shyamasundar, R.K., Agarwal, S.: Article: Clustered checkpointing
and partial rollbacks for reducing conflict costs in stms. International Journal of
Computer Applications 1(22) (February 2010) 80–85
\bibitem{monika1}
 Gupta, M., Shyamasundar, R.K., Agarwal, S. Automatic checkpointing and partial
rollback in software transaction memory (January 2012) US Patent 20110029490.
% \bibitem{CaPR}
%  M Gupta, R K Shyamasundar, S Agarwal, “CaPR: Automatic Checkpointing and Partial Rollback Algorithm for STM”.
\bibitem{HerlWing:1990:TPLS}
  M. Herlihy and J. M. Wing. ``Linearizability: a correctness condition
for concurrent objects'', \emph{ACM Transactions on Programming
Languages and Systems}, 12(3):463–492, June 1990. 
% \bibitem{serial}
%  T. Riegel, P. Felber, and C. Fetzer, ``A lazy snapshot algorithm with
% eager validation'', In Proceedings of the \emph{20th International Symposium
% on Distributed Computing (DISC’06)}, 2006.
% \bibitem{strict}
%  P. A. Bernstein and N. Goodman, ``Multiversion concurrency control—
% theory and algorithms'', \emph{ACM Transactions on Database Systems},
% 8(4):465–483, 1983.
% \bibitem{snapshot}
%  Torvald Riegel, Christof Fetzer, and Pascal Felber, ``Snapshot isolation for software trans-
% actional memory'', In \emph{TRANSACT ’06: 1st Workshop on Languages, Compilers, and Hardware
% Support for Transactional Computing}, June 2006.
\bibitem{GuerKap:2008:PPoPP}
  R. Guerraoui and M. Kapalka, ``On the correctness of transac-
tional memory'', In Proceedings of the \emph{13th ACM SIGPLAN
Symposium on Principles and practice of parallel program-
ming, PPoPP ’08}, pages 175-184. ACM, 2008
% \bibitem{RBT}
%  D. Dice, O. Shalev, et al, ``Transactional locking II'', In DISC’06: Pro-
% ceedings of the \emph{20th International Symposium on Distributed Computing}.
% March 2006.
% \bibitem{hash}
%  V. J. Marathe, M. F. Spear, et al, ``Lowering the overhead of nonblocking
% software transactional memory'', In \emph{TRANSACT: First ACM SIGPLAN
% Workshop on Languages, Compilers, and Hardware Support for Transactional Computing}, 2006.

% \bibitem{stmbench7}
%  Rachid Guerraoui, Michal Kapalka, and Jan Vitek,
% ``Stmbench7: a benchmark for software transactional
% memory'', \emph{SIGOPS Oper. Syst. Rev.}, 41(3):315-324, 2007.
% \bibitem{splash2}
%  S. C. Woo, M. Ohara, et al, ``The SPLASH2 Programs: Characterization
% and Methodological Considerations'', In Proceedings of the \emph{22nd Interna-
% tional Symposium on Computer Architecture}, pp. 24-36. June 1995.
% \bibitem{specomp}
%  Standard Performance Evaluation Corporation, SPEC OpenMP Bench-
% mark Suite. http://www.spec.org/omp.
% \bibitem{bioparallel}
%  A. Jaleel, M. Mattina, et al, ``Last level cache (llc) performance of data
% mining workloads on a cmp - a case study of parallel bioinformatics
% workloads'', \emph{The Twelfth
% International Symposium on High-Performance Computer Architecture}, 2006, pp. 88–98, 11-15 Feb. 2006. ISSN 1530-
% 0897.
% \bibitem{minebench}
%  R. Narayanan, B. Ozisikyilmaz, et al, ``Minebench: A benchmark suite
% for data mining workloads'', \emph{2006 IEEE
% International Symposium on Workload Characterization}, pp. 182–188, Oct. 2006.
% \bibitem{stamp}
%  Chi Cao Minh, JaeWoong Chung, Christos Kozyrakis,
% and Kunle Olukotun, ``STAMP: Stanford transactional
% applications for multi-processing'', In
% \emph{IISWC ’08: Proceedings of The IEEE International Symposium on
% Workload Characterization}, September 2008.
\bibitem{wali}
M. M. Waliullah and P. Stenstrom. Intermediate
checkpointing with conflicting access prediction in
transactional memory systems. In IPDPS, pages 1-11.IEEE Computer Society, 2008
\bibitem{alice}
Porfirio Alice et. al. Transparent Support for Partial Rollback in Software Transactional Memories, Euro-Par 2013 Parallel Processing, 2013
\bibitem{KR:2011:OPODIS}
Petr Kuznetsov and Srivatsan Ravi. On the cost of concurrency in transactional memory. In
OPODIS, pages 112-127, 2011.
\bibitem{AttHill:TCS:SingMult:2012}
Hagit Attiya and Eshcar Hillel. A single-version stm that is multi-versioned permissive. Theory
Comput. Syst., 51(4):425-446, 2012.
\bibitem{tm-book}
Rachid Guerraoui and Michal Kapalka. Principles of Transactional Memory,Synthesis Lectures
on Distributed Computing Theory. Morgan and Claypool, 2010.
\bibitem{CIR11}
Tyler Crain, Damien Imbs, and Michel Raynal. Read invisibility, virtual world consistency and
probabilistic permissiveness are compatible. In ICA3PP (1), pages 244–257, 2011.
\bibitem{ImbsRay:2008:OPODIS}
Damien Imbs and Michel Raynal. A lock-based stm protocol that satisfies opacity and progressiveness. 
In OPODIS ’08: Proceedings of the 12th International Conference on Principles of
Distributed Systems, pages 226–245, Berlin, Heidelberg, 2008. Springer-Verlag.
\bibitem{WeiVoss:2002:Morg}
Gerhard Weikum and Gottfried Vossen. Transactional Information Systems: Theory, Algorithms,
and the Practice of Concurrency Control and Recovery. Morgan Kaufmann, 2002.

\end{thebibliography}

